Unified Characterization and Precoding for Non-Stationary Channels

Modern wireless channels are increasingly dense and mobile making the channel highly non-stationary. The time-varying distribution and the existence of joint interference across multiple degrees of freedom (e.g., users, antennas, frequency and symbols) in such channels render conventional precoding sub-optimal in practice, and have led to historically poor characterization of their statistics. The core of our work is the derivation of a high-order generalization of Mercer's Theorem to decompose the non-stationary channel into constituent fading sub-channels (2-D eigenfunctions) that are jointly orthogonal across its degrees of freedom. Consequently, transmitting these eigenfunctions with optimally derived coefficients eventually mitigates any interference across these dimensions and forms the foundation of the proposed joint spatio-temporal precoding. The precoded symbols directly reconstruct the data symbols at the receiver upon demodulation, thereby significantly reducing its computational burden, by alleviating the need for any complementary decoding. These eigenfunctions are paramount to extracting the second-order channel statistics, and therefore completely characterize the underlying channel. Theory and simulations show that such precoding leads to ${>}10^4{\times}$ BER improvement (at 20dB) over existing methods for non-stationary channels.

==> KLT_precoding.tex <==
\section{KLT based precoding}
\label{sec:klt_precoding}
\subsection{Optimization}
Equation~\ref{eq:argmin} aims to minimize the space-time-frequency interference, denoted as $\epsilon(x)$
\begin{equation}
\epsilon(x) = \sum_{u} \sum_{k} \sum_{p}||s(u,k,p) - \sum_{n=1}^N x_n \sigma_n(u,k,p)||^2
\end{equation}

Sum $\sigma_n(u,k,p)$ along eigen dimension. Then by KLT decompostion, we can get the eigen basis (eigenfunctions) of $\{ \sigma_n\}$
\begin{align}
    A(u,k,p) & {=} \sum_{n=1}^N \sigma_n(u,k,p) \nonumber\\
    &{=} \sum_{j}^J e_j \phi_j(u,k,p) \nonumber 
\end{align}

Then $\sigma_n$ can be represented as
\begin{align}
   &\sigma_n(u,k,p) {=} \sum_{j}^J e_{n,j} \phi_j(u,k,p) \quad \text{where,} \quad \nonumber\\
    &e_{n,j} = \sum_u \sum_k \sum_p \sigma_n(u,k,p) \phi_j(u,k,p)
\end{align}

$\epsilon(x)$ can be rewritten as

\begin{align}
    & \epsilon(x) {=} \sum_u \sum_k \sum_p ||s(u,k,p) - \sum_{n}^N x_n \sum_j^J e_{n,j} \phi_j(u,k,p)||^2 \nonumber\\
    & {=} \sum_u \sum_k \sum_p ||s(u,k,p) - \sum_j^J \sum_{n}^N x_n e_{n,j} \phi_j(u,k,p)||^2 \nonumber\\
    & {=} \sum_u \sum_k \sum_p \{ ||s(u,k,p)||^2 - 2\sum_j^J \sum_{n}^N x_n e_{n,j} \phi_j(u,k,p) \nonumber\\
    & {\cdot} s(u,k,p) + \sum_j^J \sum_{n}^N \sum_{j'}^J \sum_{n'}^N x_n x_{n'} e_{n,j} e_{n',j'} \phi_j(u,k,p) \nonumber\\
    & {\cdot} \phi_{j'}(u,k,p) \} \nonumber \\
    & {=} e_{s,s} - 2\sum_j^J \sum_{n}^N x_n e_{n,j} e_{s,j} + \sum_j^J \sum_{n}^N x_n^2 e_{n,j}^2 \nonumber \\
    & {+} \sum_j^J \sum_{n}^N \sum_{n'\neq n}^N x_n x_{n'} e_{n,j} e_{n',j}  \nonumber \\ 
\end{align}
where $e_{s,s} = \sum_u \sum_k \sum_p ||s(u,k,p)||^2$ is the energy of $S$, and $e_{s,j} = \sum_u \sum_k \sum_p s(u,k,p) \phi_j(u,k,p)$ is the projection of $S$ onto $\phi_j$.

To find the minimum $\epsilon(x)$, let the partial derivative of $\epsilon(x)$ with respect to $x_n$ be zero
\begin{align}
    \pdv{\epsilon(x)}{x_n} & {=} - 2\sum_j^J e_{n,j} e_{s,j} + 2 \sum_j^J x_n e_{n,j}^2 \nonumber \\
    & {+} 2 \sum_j^J \sum_{n'\neq n}^N x_{n'} e_{n,j} e_{n',j} = 0 \nonumber \\ 
\end{align}

Then $x_n$ is
\begin{align}
    x_n & {=} \frac{\sum_j^J e_{n,j} e_{s,j} + \sum_j^J \sum_{n'\neq n}^N x_{n'} e_{n,j} e_{n',j} }{\sum_j^J e_{n,j}^2} \nonumber \\
    & {=} \frac{\sum_j^J e_{s,n} e_{j,j} + \sum_j^J \sum_{n'\neq n}^N x_{n'} e_{n,n'} e_{j,j} }{\sum_j^J e_{n,n} e_{j,j}} \nonumber \\
    & {=}  \frac{e_{s,n} + \sum_{n'\neq n}^N x_{n'} e_{n,n'} }{e_{n,n}} \nonumber 
\end{align}
where $e_{n,n} = \sum_u \sum_k \sum_p ||\sigma_n(u,k,p)||^2$ is the energy of $\sigma_n$. $e_{s,n}$ and $e_{n,n'}$ are the projection of $S$ and $\sigma_n'$ onto $\sigma_n$, respectively. It's an iterative optimization. 

Specifically, if $\{ \sigma_n \}_n^N$ are orthogonal basis, i.e. $e_{n,n'} = \sum_u \sum_k \sum_p \sigma_n(u,k,p) \sigma_{n'}(u,k,p) = 0 \quad \text{for} \quad n' \neq n$, we have 
\begin{align}
    x_n & {=} \frac{ e_{s,n}}{e_{n,n}} \nonumber \\
\end{align}

\noindent
\textbf{KLT precoding}: 
Decompose the mixed space-time-frequency response $z(m,l,p)$ to get eigenfunction $\{ \phi_n \}$. We can not ensure the projection $\{\sigma_n\}$ are orthogonal to fully cancel interference (here, interference means $\epsilon(x)$).  

Interference: minimize $\epsilon(x)$ but can not ensure $\epsilon(x) = 0$. (in some cases, the combination of non-orthogonal $\{\sigma_n\}$ can achieve $\epsilon(x) = 0$.)

Diversity: fully use.

Complexiy: low.

If KLT precoding can design eigenfunctions $\{ \phi_n \}$ that can directly get orthogonal $\{\sigma_n\}$, it would be optimal with respect to interference, diversity and complexity.

\note{
\noindent
\textbf{BD-KLT precoding}:
Find $N=U*K*P$ eigenfunctions, each eigenfuntion is the zero space of the response of all users over all time and all carriers except for the response at desired $(u,k,p)$, i.e.,
\begin{align}
    & \sum_m \sum_l \sum_q h(u,k,p;m,l,q) * \phi_n^* (m,l,q) \nonumber\\
    &{=} \left\{\begin{array}{ll}
    \sigma_n(u,k,p) & \text { if } n = u*P*K+p*K+k \\
    0 & \text { otherwise}
    \end{array}\right.
\end{align}

Then we can get $N=U*K*P$ orthogonal basis $\{\sigma_n\}$, where $N$ is greater or equal to the rank of $S$. So we must achieve $\epsilon(x) = 0$.  

Interference: $\epsilon(x) = 0$

Diversity: not use other channels gain

Complexiy: low

\noindent
\textbf{THP-KLT precoding}:
Using GS method to get the eigenfunctions of each $h(u,k,p;m,l,q)$. For example, by GS we get
\begin{align}
    &h(1,1,1;m,l,q) = \sigma_1(1,1,1) \phi_1(m,l,q) \nonumber\\
    &h(1,1,2;m,l,q) = \sigma_1(1,1,2) \phi_1(m,l,q) + \sigma_2(1,1,2) \phi_2(m,l,q)
\end{align}

Then we can get $x_n$ by
\begin{align}
    &x_1 = \frac{s(1,1,1)}{\sigma_1(1,1,1)} \nonumber\\
    &x_2 = \frac{s(1,1,2) - x_1 \sigma_1(1,1,2)}{\sigma_2(1,1,2)}
\end{align}

Interference: $\epsilon(x) = 0$

Diversity: fully use

Complexiy: high
}

\subsection{Error analysis}
\note{
\noindent
Waiting for extension.
}
% \begin{equation}
% \mathbf{H}=\sum_{n} \sum_{k} \sum_{m} \sum_{l} \eta_{n, k}^{m, l} \mathbf{\phi}_{n T_{0}, k F_{0}}^{m \tau_{0}, l \nu_{0}}
% \end{equation}

% The ambiguity function of the $x$, $A_{x}(t, f; \tau, \nu)$ is defined by 


% \begin{equation}
% \begin{aligned}
% A_{x}(t, f; \tau, \nu) &=\left\langle x(t), x(t-\tau) e^{j 2 \pi (f-\nu) t}\right\rangle \\
% &=\int x(t) x^{*}(t-\tau) e^{-j 2 \pi (f - \nu t)} d t
% \end{aligned}
% \end{equation}
In this section, we investigate the performance and limitations of the precoding algorithm using eigenfunctions obtained from section \ref{sec:AE}.

\noindent
\inred{Zhibin: Reformulate Lemmas 1-3 to be consistent with Section III.}

\begin{lemma}
\label{lemma:1}
Let $\{\hat{\phi}_n\}_{n=1}^N$ be the \note{eigenfunctions corresponding to the obsolete CSI/ prediction}, then the precoded signal {X} can be decomposed by
\begin{equation}
\begin{aligned}
X &=\sum_{n}^{N} x_{n} \hat{\phi}_{n} \\
&=\sum_{n}^{N} \langle\phi_{n}, \hat{\phi}_{n} \rangle \phi_{n} x_{n}+\langle \Delta \phi_{n}, \hat{\phi}_{n} \rangle \Delta \phi_{n} x_{n}
\end{aligned}
\end{equation}\
where, $\phi_n$ is $n^{th}$ eigenfuntion of real channel.  $\Delta \phi_n $ is the prediction error and orthogonal to $\phi_n$ , and 
\begin{equation}
    \langle \phi_n ,\phi_m \rangle = \int \phi_n \phi_m d t
\end{equation}
denotes the inner product. Where we have $\langle \phi_n ,\phi_n \rangle = 1, \langle \Delta \phi_n ,\phi_n \rangle = 0, \langle \phi_n ,\phi_m \rangle = 0 ~ \text{for} ~ n \neq m$, and

\begin{equation}
    \langle \hat{\phi}_n ,\hat{\phi}_n \rangle ^2 = \langle \phi_n ,\hat{\phi}_n \rangle ^2 + \langle \Delta \phi_n ,\hat{\phi}_n \rangle ^2
\end{equation}
\end{lemma}
The proof is provided in Appendix~\ref{app:lemma_1}.

\begin{lemma}
\label{lemma:2}
The eigenfunctions prediction error $\Delta\Phi = \{\Delta \phi_n\}_{n=1}^N$ can be equivalent to CSI error $\Delta H = \sum_{n=1}^{N} \Delta \sigma_n \phi_n$ where
\begin{equation}
\Delta \sigma_{n}=\frac{\sigma_{n} \sum_{m} x_{m} \langle \phi_{n}, \Delta \phi_{m}\rangle}{x_{n}}
\end{equation}
\end{lemma}

The proof is provided in Appendix~\ref{app:lemma_2}.

\begin{lemma}
\label{lemma:3}
Given CSI error $\Delta H$, the expected transmit error is bounded by 
\begin{equation}
\sigma_{N} \min \left(x_{1}\cdots x_{N}\right) E_{\Delta} \leqslant E[ \Delta H \tilde{X} ]\leqslant \sigma_{1} \max \left(x_{1}\cdots x_{N}\right) E_{\Delta},
\end{equation}
where, $E_{\Delta}=\int \Delta \Phi \cdot \Phi$. $\tilde{X}$ is the transmitted signal precoded by perfect eigenfunctions.
\end{lemma}
The proof is provided in Appendix~\ref{app:lemma_3}.


\note{The objective function can choose minimizing MSE $E\{|\Delta H \tilde{X}|^{2}\}$ or maximizing the SINR}

\begin{equation}
\argmax_{\{x_{n}\} \{\hat{\phi}_{n}\}} \mathrm{SINR}=\frac{E\{|H \tilde{X}|^2\}}{\sigma_W^{2}+E\{|\Delta H \tilde{X}|^2\}}
\end{equation}








\begin{comment}


The received signal can be written as
\begin{equation}
Y = HX + W.    
\end{equation}

Let $E\{W^2\} = \sigma^2_W$. We have
\begin{equation}
\begin{aligned}
& E\{H X\} \\
=& \int \sum_{n}^{N} \sigma_{n} \phi_{n} \cdot \sum_{m}^{N} X_{m}(\langle \hat{\phi}_{m}, \phi_{m} \rangle \phi_{m}+\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \Delta \phi_{m}) d t\\
=& \sum_{n}^{N} \int \sigma_{n} \phi_{n} \cdot x_{n}(\langle\phi_{n}, \hat{\phi}_{n}\rangle \phi_{n}+\langle\phi_{n}, \hat{\phi}_{n} \rangle \Delta \phi_{n})\\
+&\sum_{m \neq n}^{N} \sigma_{n} \phi_{n} \cdot x_{m}(\langle\phi_{m}, \hat{\phi}_{n}\rangle \phi_{m}+\langle\Delta \phi_{n}, \hat{\phi}_{m}\rangle \Delta \phi_{n}) d t\\
=& \sum_{n}^{N}\{\sigma_{n} x_{n}\langle \phi_{n} \hat{\phi}_{n}\rangle \cdot \int \phi_{n} \phi_{n} d t +\sigma_{n} x_{n}\langle\Delta \phi_{n}, \hat{\phi}_{n}\rangle \cdot\int \phi_{n} \Delta \phi_{n} d t \\
+&\sum_{m \neq n}^{N}[\sigma_{n} x_{m}\langle\phi_{m}, \hat{\phi}_{m}\rangle \cdot \int \phi_{n} \phi_{m} d t+\sigma_{n} x_{m}\langle \Delta \phi_{m} \hat{\phi}_{m} \rangle \int \Delta \phi_{m} \phi_{n} d t]\} \\
=& \sum_{n}^{N}[\sigma_{n} x_{n}\langle\phi_{n}, \hat{\phi}_{n}\rangle+\sum_{m}^{N} \sigma_{n} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \int \phi_{n} \Delta \phi_{m} d t]\\
=& \sum_{n}^{N}[\sigma_{n} x_{n}\langle\phi_{n}, \hat{\phi}_{n}\rangle+\sum_{m}^{N} \sigma_{n} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \langle \phi_{n}, \Delta \phi_{m} \rangle]\\
\end{aligned}
\end{equation}

We also have 

\begin{equation}
\begin{aligned}
E\{H \tilde{X}\} &=\int \sum_{n}^{N} \sigma_{n} \phi_{n}  \cdot \sum_{m}^{N} x_{m} \phi_{m} d t \\
&=\sum_{n} \sigma_{n} x_{n} .
\end{aligned}
\end{equation}

Thus the MSE caused by imperfect CSI is given by
\begin{equation}
\begin{aligned}
& E\{|\Delta H \tilde{X}|^{2}\}= E\{|H \Delta X|^{2}\} = E\{|H X-H \tilde{X}|^{2}\}\\
=&E\{| \sum _ { n } [ \sigma_{n} x_{n} ( \langle\phi_{n}, \hat{\phi}_{n}\rangle -1) +\sum_{m}^{N} \sigma_{n} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \langle\Delta \phi_{m}, \phi_{n}\rangle ]|^{2} \} \\
=&E\{|\sum_{n}^{N} \sigma_{n}[x_{n}(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1) +\sum_{m}^{N} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle \Delta \phi_{m}, \phi_{n}\rangle]|^{2}\}\\
=& \sum_{n}^{N} E\{\sigma_{n}^{2}|x_{n}(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1)+\sum_{m}^{N} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_{n}\rangle|^{2}\} \\
&+\sum_{n^{'} \neq n}^{N} E\{\sigma_{n^{'}} \sigma_{n} \cdot |\cdots|^{2}\},
\end{aligned}
\end{equation}

where $|\cdots|^2$ is the residual part, which is uncorrelated with $\sigma_n$. 
Meanwhile $E \{ \sigma_n \sigma_{n^{'}} \} = 0$ for $n \neq n^{'}$ , so the last item is $0$. Then We have

\begin{equation}
\begin{aligned}
&E\{|\Delta H \tilde{X}|^{2}\}\\
=& \sum_{n}^{N} \sigma_{n}^{2} E\{|x_{n}(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1)+\sum_{m}^{N} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_n \rangle|^{2}\} \\
=& \sum_{n}^{N} \sigma_{n}^{2} E\{| x_{n}[(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1) + \langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_{n}\rangle]\\
&+\sum_{m \neq n} x_{m}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle \Delta \phi_{m}, \phi_{n}\rangle|^{2}\}\\
=&\sum_{n}^{N} \sigma_{n}^{2} E\{ x_{n}^{2}[(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1)+ \langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_{n} \rangle]^{2}\\
&+\sum_{m \neq n}^{N} x_{m}^{2}(\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle\langle\Delta \phi_{m}, \phi_{n} \rangle)^{2}\} + \sum_{n^{'} \neq n}E \{x_{n^{'}} x_{n} \cdot |\cdots|^{2}\}.
\end{aligned}
\end{equation}

Also, $|\cdots|$ is uncorrelated with $x_n$ and $E \{ x_n x_{n^{'}} \} = 0$ for $n \neq n^{'}$. So, we have
\begin{equation}
\begin{aligned}
&E\{|\Delta H \tilde{X}|^{2}\}\\
=&\sum_{n}^{N} \sigma_{n}^{2} \{ x_{n}^{2}[(\langle\phi_{n}, \hat{\phi}_{n}\rangle-1) + \langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle \langle\Delta \phi_{m}, \phi_{n} \rangle]^{2}\\
&+\sum_{m \neq n}^{N} x_{m}^{2}\langle\Delta \phi_{m}, \hat{\phi}_{m}\rangle ^2 \langle\Delta \phi_{m}, \phi_{n} \rangle^{2}\}.
\end{aligned}
\end{equation}

\note{The objective function can choose minimizing MSE $E\{|\Delta H \tilde{X}|^{2}\}$ or maximizing the SINR}

\begin{equation}
\argmax_{\{x_{n}\} \{\hat{\phi}_{n}\}} \mathrm{SINR}=\frac{E\{|H \tilde{X}|^2\}}{\sigma_W^{2}+E\{|\Delta H \tilde{X}|^2\}}
\end{equation}

% \begin{equation}
% E\{||H X||^2\} = \iiiint \mathcal{C}_{\mathbf{H}}(t, f ; \tau, \nu) \cdot \sigma^2 |\phi|^2 \mathrm{d} t \mathrm{d} f \mathrm{d} \tau \mathrm{d} \nu
% \end{equation}
\end{comment}


\note{
Objectives:\\
1. Model and solve the optimization problem for one criteria (MSE, SINR, EE, BER, etc.) under imperfect CSI/predicted eigenfunctions.\\
2. Predict eigenfunctions (Take the time-memory advantages of KLT over SVD).\\
3. Design autoencoder.}

\begin{theorem}
\note{Generalized precoding theorem: The proposed method is an optimal precoding approach for any channel / better than other methods.}

\end{theorem}


\begin{corollary}
\label{corollary_1}
For SU-MIMO, given perfect time series CSI $H(t) =\sum_{n=1}^{N} \sigma_n \phi_n (t)$, the expected capacity can be achieved by KLT precoding $X(t) = \sum_{n=1}^{N} x_n \phi_n(t)$, where $\{x_n\}_{n=1}^N$ is designed by water filling algorithm.
\end{corollary}

The proof is provided in Appendix [].







==> related.tex <==
% \newpage
\section{Related Work}
\label{sec:related}

% The related 

\noindent
\textbf{Neural Network based Transceivers:}
% Deep Learning has emerged as a versatile tool for physical layer communication due to its proficiency in systems with model and algorithm deficit \cite{simeone2018very}, and has been used to replace individual blocks in communication systems for optimized performance for a given dataset. 
Despite the increasing interest of DL to replace classical communication systems, these systems have come at the cost of increased training time and model complexity and have at best approached the error rate of classical methods \cite{kim2018communication,gruber2017deep}. 
% The stringent requirements on reliability and achievable throughput in xG propagation environments demand wireless communication systems that achieve provable performance guarantees over a variety of channels. 
So far, much of the effort has been focused on replacing individual blocks \cite{tan2018improving,klautau2018detection} or the end-to-end chain~\cite{DeepSig2,aoudia2018endtoend} in classical transceivers using ``black-box" neural networks to achieve a target error rate for a specific dataset.
These fixed function implementations that fits a particular dataset cannot be generalized to other scenarios.
This has limited the wide-spread practical adoption of neural network based communication systems, due to their lack of explainability \cite{guo2020explainable6G} and performance guarantees on the error rate or the complexity (training or hardware complexity). 
% Fueled by the promising results shown in other domains, wireless researchers have adopted a learning based approach in order to tame the stochasticity of the wireless channel. 
In order to make wireless communications explainable, we take the first step towards understanding what happens inside a NN-based receiver that eventually performs equivalent to a classical receiver. 
We use this knowledge to derive tight bounds on the BER of NN-based receivers that achieve strict communication guarantees essential for practical adaptation. 
% Moreover, we de


\noindent
\textbf{Explainable Neural Networks:}
% The very first results have demonstrated the universal approximation of DNNs, that is, any continuous function defined on a compact set can be approximated at any precision using a DNN [20], [21]. Recently, some effort has been made to analyze how the structural properties of DNNs, mainly depth and width, contribute to their powerful capability of modeling functions, i.e., expressive power of DNNs [22]–[24]. These works converge to a similar conclusion that the expressive power of a DNN grows exponentially with its depth, which is compelling and provides some meaningful theoretical insights into superior performance of DNNs in practice. However, previous research seldom involves with the theoretical interpretation on the performance of DL embedded communication systems.
% A majority of DL approaches rely on a black-box approach to replace classical transceivers with neural networks and achieve comparable performance, while lacking guarantees or the robustness to generalize beyond the trained data.
% We outline the literature that have attempted to move away from this black-box data-driven approach by primarily relying on model-driven techniques.
% The end-to-end autoencoder-based system has been extended to multi-user communication over interference channels, OFDM systems with multipath channels in \cite{felix2018ofdmautoencoder}. In \cite{ye2018channel}, the purely data-driven DL method has been used in transceiver optimization without using accurate CSI. 
The explainability of neural network based transceivers is very rare in the literature, attributed primarily due to their black-box implementation. 
Of particular relevance here, is the literature that instead rely on model-driven techniques to avoid the black box approach, and incorporate expert knowledge into autoencoder-based communication systems with the radio transformer network~\cite{o'shea2016radio} and the OFDM-autoencoder~\cite{felix2018ofdmautoencoder}. 
\cite{felix2018ofdmautoencoder} combines an autoencoder with a classical OFDM system to inherit its advantages, including robustness to synchronization errors and multipath equalization.
The model-driven OFDM receiver in~\cite{gao2018comnet} combines DL with expert knowledge and implements two subnets for channel estimation and symbol detection modular structure similar to classical systems. 
% involves two subnets for channel estimation and symbol detection which are combined in a block-by-block manner similar to classical systems. 
% Model-driven DL shows a competitive performance with data-driven approaches but with a lower number of trainable variables than the black box architecture. 
However these approaches are limited by the flexibility and accuracy of the underlying model and the trained weights, which limits their applicability to specific channel conditions. 
% This limits the generality of these approaches to a wide variety of channel conditions and limit their ability to adapt online to changes in channel conditions. 
% \cite{qiang2020deep} present initial interpretation of neural networks for channel estimation tasks, that approaches the performance of classical channel estimators.  
In contrast, we achieve guarantees on the performance of data-driven NN-based receivers by explaining their internal mechanisms and deriving their structure that achieves equivalence to MAP receiver.
This allows for low-complexity NN-based receivers that are robust to various channels.  
% \note{To be included: 
% 1/2-1 column.}





% \newpage

==> system.tex <==
\section{System Design}
\label{sec:system}

\begin{comment}
\begin{corollary}
\label{col:svdfortensors}
The tensor form of theorem~\ref{thm:svdforfunctions}: Let $\mathbf{K}$ be $P$ order tensor with rank $N$, obtained by Kronecker product of $P$ vectors $\mathbf{K} = \mathbf{x}_1 \otimes \mathbf{x}_2 \otimes,...,\otimes \mathbf{x}_P$. Then $\mathbf{K}$ can be expressed by
\begin{equation}
\mathbf{K} = \sum_n^N \sigma_n \mathbf{u}_n^{(1)}\otimes \mathbf{u}_n^{(2)} \otimes,...,\otimes \mathbf{u}_n^{(P)}
\end{equation}
where $\sigma_n$ is singular value. $\{\mathbf{u}_n^{(p)}\}_n$ are eigenvectors.
Specially, when $P$ = 2, it's the same with SVD.
\end{corollary}
\end{comment}


\subsection{CSI Processing \& Eigendecomposition}
\label{sec:AE}


\begin{definition}
Given a $k^2$ order tensor $\mathcal{A}(A_{j_1,j_2,\cdots,j_k})$, where $A_{j_1,j_2,\cdots,j_k}$ is the $k$ order cell. If
\begin{equation}
    \mathcal{A}(\langle A_{j_1,j_2,\cdots,j_k}, T_i\rangle_{\mathrm{F}}) = \lambda_i T_i
\end{equation}
where $\langle\mathbf{\cdot}, \mathbf{\cdot}\rangle_{\mathrm{F}}$ is \textit{Frobenius inner product}. Then $T_i$ is a $k$ order eigentensor, where eigentensor $T_i$ is orthonormal. 
\begin{align}
    &\langle T_i, T_i\rangle_{\mathrm{F}} = 1 \nonumber \\ 
    &\langle T_i, T_j\rangle_{\mathrm{F}} = 0 \quad \text{for }\quad i \neq j \nonumber \\ 
\end{align}

\begin{comment}
    \begin{equation}
    \langle\mathbf{A}, \mathbf{B}\rangle_{\mathrm{F}}=\sum_{i, j} \overline{A_{i j}} B_{i j}=\operatorname{Tr}\left(\overline{\mathbf{A}^{T}} \mathbf{B}\right) \equiv \operatorname{Tr}\left(\mathbf{A}^{\dagger} \mathbf{B}\right)
    \end{equation}
\end{comment}

\end{definition}

\begin{corollary}
\label{col:svdfortensors}
The tensor form of corollary~\ref{col:svdforNSchannel}: 
Denote non-stationary jointly Gaussian channel as six order tensor $\textbf{H}$. The entry $H(u,k,p; m,l,q)$ denotes the space-time-frequency response of user $u$ at time $k$ (period of k is OFDM symbol duration time) and carrier $q$.
$\textbf{H}$ can be expressed as 
\begin{equation}
    \textbf{H} = \sum_n^N \sigma_n \textbf{A}_n \otimes \textbf{B}_n
\end{equation}
where \textbf{A} and \textbf{B} are both three order tensors and have entry $A(u,k,p)$ and $B(m,l,q)$, respectively.
\end{corollary}


\begin{theorem}
% The proposed autoencoder provides a computationally efficient and correct decomposition of the channel into KLT eigenfunctions.
\inred{Need modify} Training a deep autoencoder by sequentially feeding  each column of hankel matrix represented as $\textbf{x}$ (or each lateral slice of hankel tensor) with the following regularized loss, 
% $\mathcal{L}{=}\mathcal{J}{+}\Omega$, where $\mathcal{J}{=}\|\textbf{x}-\hat{\textbf{x}}\|^2$ ($\textbf{x}$ represents each column of the hankel matrix $\textbf{U}$ which is used to train the AE) and $\Omega$ as defined below,
\begin{align*}
% \small
\mathcal{L}&{=}\mathcal{J}{+}\Omega, \quad \text{where}, \quad \mathcal{J}{=}\|\textbf{x}-\hat{\textbf{x}}\|^2\\
% \operatorname{L}_{KLT}(\Phi)=-\sum_{i=1}^{m} \phi_{i}^{\mathrm{T}} Q \phi_{i}+ \gamma \sum_{i=1}^{m}\left(\phi_{i}^{T} \phi_{i}-1\right)+ \beta \sum_{i=1}^{m} \sum_{j=1}^{i-1} \phi_{i}^{T} \phi_{j}+ \eta \sum_{i=1}^{m} \sum_{j=1}^{i-1}  \phi_{i}^{T} Q \phi_{j}
% \Omega(\boldsymbol{W}_{dec})= \lambda \left(\sum_{i{=}1}^{M}\left(w_{i}^{H} \phi_{i}-1\right)+ \sum_{i=1}^{M} \sum_{j=1}^{i-1} \phi_{i}^{H} \phi_{j}+ \sum_{i=1}^{M} \sum_{j=1}^{i-1}  \phi_{i}^{H} \mathbf{R_{\mathbf{xx}}} \phi_{j} \right)
\Omega(\boldsymbol{W}_{dec})&{=} \lambda \left([\boldsymbol{W}_{dec}^H\boldsymbol{W}_{dec}-\boldsymbol{I}] + \boldsymbol{W}_{dec}^H\mathbf{R_{\mathbf{xx}}}\boldsymbol{W}_{dec}\right)
\end{align*}
ensures that the weights of the trained AE, $W_{enc}^T=W_1^TW_2^T{\ldots}W_d^t=W_{dec}\rightarrow \mathbf{\Phi}$.
\end{theorem}

The proof is presented in Appendix.

\begin{comment}
Transmitting the unprecoded data $S$, we receive $y(u,k,p)$ at the receiver\footnote[1]{$\circledast_d$ denotes d-dimensional convolution.},
\begin{align}
   &y(u,k,p) {=} h(u,k,q;u,k,q)\circledast_3 s(u,k,q) \nonumber\\
   &{=} \sum_{m}\sum_{l}\sum_{q} h(u,k,p;m,l,q) s^*(u-m,k-l,p-q) \nonumber\\
   &{=}  h(u,k,p;0,0,0) s(u,k,p) \\
   &{+} \sum_{m' \neq 0} \sum_{l'\neq 0} \sum_{q' \neq 0} h(u,k,p;m',l',q') s^*(u-m',k-l',p-q')\nonumber
\end{align}
The second item is space-time-frequency interference.
\note{\noindent
Space-time-frequency interference not only includes IUI, ISI and ICI, but also includes IUI-ISI-ICI joint interference. 
Therefore, joint precoding is benefitial compared to separate precoding.
}
%
The \textit{channel correlation function} (CCF) is 
\begin{align}
    & R_h(\Delta u, \Delta k, \Delta p;\Delta m, \Delta l, \Delta q) {=} \sum_{u} \sum_{k} \sum_{p} E \{h(u,k,p;m,l,q) \\
    & {\cdot} h(u + \Delta u, k + \Delta k, p + \Delta p; m +\Delta m, l + \Delta l, q + \Delta q)\}\\
    & {=} \sum_{n}^ N \lambda_n R_{\psi_n}(\Delta u,\Delta k,\Delta p) R_{\phi_n}(\Delta m,\Delta l, \Delta q)
\end{align}

The \textit{local scattering function} (LSF) is
\begin{align}
    & C_h(u, k, p; m, l, q) {=} \sum_{u} \sum_{k} \sum_{p}R_h(\Delta u, \Delta k, \Delta p;\Delta m, \Delta l, \Delta q) \\
    & {\cdot} h(u + \Delta u, k + \Delta k, p + \Delta p; m +\Delta m, l + \Delta l, q + \Delta q)\}\\
    & {=} \sum_{n}^ N \lambda_n R_{\psi_n}(\Delta u,\Delta k,\Delta p) R_{\phi_n}(\Delta m,\Delta l, \Delta q)
\end{align}

%
Before precoding, we need to extract space-time-frequency joint orthogonal functions.
% 
The \textbf{Mix} module is to combine space-time-frequency response of all users over all moments and carriers. 
% 
\begin{equation}
z(m,l,q) = \sum_{u} \sum_{k} \sum_{p} h(u,k,p;m,l,q)
\end{equation}
% 
Through \textbf{AE-KLT}, we have eigenfunctions that are jointly orthonormal in space-time-frequency.
\begin{align}
&z(m,l,q) = \sum_{n=1}^N \sigma_n \phi_n(m,l,q), \quad \text{where,} \quad \\
&\sum_m \sum_l \sum_q \phi_n(m,l,q)\phi^*_n(m,l,q) {=} 1\\
&\sum_m \sum_l \sum_q \phi_n(m,l,q)\phi^*_{n'}(m,l,q) {=} 0 ~\text{for}~n \neq n'
\end{align}
% 
As $z(m,l,q)$ combine all $h(u,k,p;m,l,q)$, the eigenfunctions decomposed from $z(m,l,q)$ are also basis of $h(u,k,p;m,l,q)$.
\begin{equation}
h(u,k,p;m,l,q) = \sum_{n=1}^N \sigma_n(u,k,p) \phi_n(m,l,q)
\end{equation}

where, $\sigma_n(u,k,p)$ can be obtained by \textbf{Projection}
\begin{equation}
\sigma_n(u,k,p) = \sum_{m} \sum_{l} \sum_{q} h(u,k,p;m,l,q) \phi_n^*(m,l,q)
\end{equation}
\end{comment}
\subsection{Space-time-frequency Eigen-Precoding}
\begin{comment}

\textbf{Precoding} $X = W(\Sigma, \Phi; S)$ has two parts:

\noindent
\textbf{Step A:} \textbf{Minimize IUI-ISI-ICI} module is to design $\{x_n\}$ that can achieve least sum distance in space-time-frequency domain  (minimal total interference).
\begin{equation}
\label{eq:argmin}
\argmin_{\{x_n\}} \sum_{u} \sum_{k} \sum_{p}||s(u,k,p) - \sum_{n=1}^N x_n \sigma_n(u,k,p)||^2
\end{equation}
\note{\noindent
Given tensor S and the tensor set {$\Sigma_n(u,k,p)$}, how to combine {$\Sigma_n(u,k,p)$} with the coefficients $x_n$ to get the minimal distance from S (interference). If it is one dimension (vector), it's easy to cancel the interference (depends on the rank of basis). Higher order, harder to cancel all interference.

The combination problem is suitable to NN.

Minimizing BER criteria: Let $r(u,k,p) = \sum_{n=1}^N x_n \sigma_n(u,k,p)$, and given noise variance $\sigma_0^2$. If a QAM symbol $s(u,k,p)$ has decision region $D(u,k,p)$, and let $C\{r(u,k,p), \sigma_0\}$ denotes a circle area with center $r(u,k,p)$ and radius $\sigma_0$,  the minimizing BER criteria would be

\begin{align}
& \argmax_{\{x_n\}} \sum_u \sum_k \sum_p D(u,k,p) \cap C\{r(u,k,p), \sigma_0\} \quad \text{where,} \quad\\
& r(u,k,p) {=} \sum_{n=1}^N x_n \sigma_n(u,k,p)
\end{align}
}

\noindent
\textbf{Step B:}
The \textbf{construction} module constructs $X$ by linear combining the eigenfunctions with the designed coefficients $\{x_n\}$.
% 
\begin{equation}
x(u,k,p) = \sum_{n=1}^N x_n \phi_n(m-u,l-k,q-p)
\end{equation}
Transmitting the precoded data $X$, we receive $y'(u,k,p)$ at the receiver given by, 
% 
\begin{align}
    &y'(u,k,p) {=} h(u,k,p;u,k,p) \circledast_3 x(u,k,p) + w(u,k,p)\nonumber\\
    &{=} \sum_{m} \sum_{l} \sum_{q} h(u,k,p;m,l,q) x^*(u-m,k-l,p-q) \nonumber\\
    & {+} w(u,k,p)\nonumber \nonumber\\
    & {=} \sum_{m} \sum_{l} \sum_{q} \sum_{n=1}^N \sigma_n(u,k,p) \phi_n(m,l,q) \nonumber \\  
    &{\cdot} \sum_{n'=1}^N x_{n'} \phi_{n'}^*(m,l,q) {+} w(u,k,p) \nonumber\\
    & {=} \sum_{n=1}^N x_{n} \sigma_n(u,k,p) \sum_{m} \sum_{l} \sum_{q}  \phi_n(m,l,q) \phi_{n}^*(m,l,q) \nonumber\\
    & {+} {\sum_{n'\neq n}^N x_{n'} \sigma_n(u,k,p) \sum_{m} \sum_{l} \sum_{q}} \phi_n(m,l,q) \phi_{n'}^*(m,l,q)\nonumber \\
    &{+} w (u,k,p) \nonumber\\
    & {=} {\sum_{n=1}^N} x_n \sigma_n(u,k,p){+} w (u,k,p) \nonumber
\end{align}

\end{comment}
\begin{comment}

\subsection{Performance analysis}
For non-precoding data $S$, we can get the KLT expasion:
\begin{equation}
    s(u,k,p) = \sum_n s_n \phi_n(m-u,l-k,q-p)
\end{equation}

The total interference is 
\begin{align}
&\epsilon {=} \sum_{u} \sum_{k} \sum_{p}||s(u,k,p) - \sum_{n=1}^N s_n \sigma_n(u,k,p)||^2 \\
& {\leq} \sum_{u} \sum_{k} \sum_{p}||s(u,k,p) - \sum_{n=1}^N x_n \sigma_n(u,k,p)||^2
\end{align}

\end{comment}


\begin{comment}
\begin{equation}
\begin{aligned}
\mathcal{H}(X(t)) &=\int_{0}^{T_{m}} H(t;\tau) X(t-\tau) d \tau \\
&=\int_{0}^{T_{m}} \int_{-B_{d} / 2}^{B_{d} / 2} H(\tau, \nu) X(t-\tau) e^{j 2 \pi \nu t} d \nu d \tau 
\end{aligned}
\end{equation}

Where $H(t;\tau) = [H_1^H(1, t;\tau),\cdots,H_M^H(t;\tau)]^H$. 


The eigenfunction $\phi_n(\tau,\nu)$ and eigenvalue $\lambda_n$ of $H_u(\tau,\nu)$ are defined by the eigenequation
\begin{equation}
H_u\phi_n(\tau, \nu) = \lambda_n \phi_n(\tau,\nu)
\end{equation}


By KLT, we can also get 
\begin{equation}
Z(\tau, \nu) = \sum_{n=1}^N \sigma_n \phi_n(\tau,\nu)
\end{equation}
\end{comment}

\begin{comment}
\note{Why eigenfunctions: If we have a flat fading channel H, we can transmit data through the orthogonal space of the channel to cancel ISI. We know any channel can be represented by orthogonal sine waves. So we can transmit data trough frequency space, which is OFDM. but when it comes to delay-Doppler time-varying channels. There will be interferences at frequency space. So we can find eigenfunctions jointly orthogonal at time-frequency space to cancel ISI-ICI joint interference. Expand it to space, eigenfunctions can jointly orthogonal at space-time-frequency domain and cancel IUI-ISI-ICI.}
\end{comment}


